Cell Nuclei Detection and Classification in Whole Slide Images with Transformers

Accurate and efficient cell nuclei detection and classification in histopathological Whole Slide Images (WSIs) are pivotal for digital pathology applications. Traditional cell segmentation approaches, while commonly used, are computationally expensive and require extensive post-processing, limiting their practicality for high-throughput clinical settings. In this paper, we propose a paradigm shift from segmentation to detection for extracting cell information from WSIs, introducing CellNuc-DETR as a more effective solution. We evaluate the accuracy performance of CellNuc-DETR on the PanNuke dataset and conduct cross-dataset evaluations on CoNSeP and MoNuSeg to assess robustness and generalization capabilities. Our results demonstrate state-of-the-art performance in both cell nuclei detection and classification tasks. Additionally, we assess the efficiency of CellNuc-DETR on large WSIs, showing that it not only outperforms current methods in accuracy but also significantly reduces inference times. Specifically, CellNuc-DETR is twice as fast as the fastest segmentation-based method, HoVer-NeXt, while achieving substantially higher accuracy. Moreover, it surpasses CellViT in accuracy and is approximately ten times more efficient in inference speed on WSIs. These results establish CellNuc-DETR as a superior approach for cell analysis in digital pathology, combining high accuracy with computational efficiency.

==> sections/highlights.tex <==
\begin{itemize}
    \item Introduced CellNuc-DETR, a detection-based method for efficient cell nuclei analysis in WSIs.
    \item Achieved state-of-the-art performance on PanNuke dataset for detection and classification.
    \item Validated robustness via cross-dataset evaluation on CoNSeP and MoNuSeg datasets.
    \item Demonstrated up to 10x faster inference compared to segmentation-based methods.
    \item Optimized for clinical deployment with a scalable, efficient pipeline for large WSIs.
\end{itemize}
